Vector Commitments with Efficient Updates

Dynamic vector commitments that enable local updates of opening proofs have applications ranging from verifiable databases with membership changes to stateless clients on blockchains. In these applications, each user maintains a relevant subset of the committed messages and the corresponding opening proofs with the goal of ensuring a succinct global state. When the messages are updated, users are given some global update information and update their opening proofs to match the new vector commitment. We investigate the relation between the size of the update information and the runtime complexity needed to update an individual opening proof. Existing vector commitment schemes require that either the information size or the runtime scale linearly in the number $k$ of updated state elements. We construct a vector commitment scheme that asymptotically achieves both length and runtime that is sublinear in $k$, namely $k^\nu$ and $k^{1-\nu}$ for any $\nu \in (0,1)$. We prove an information-theoretic lower bound on the relation between the update information size and runtime complexity that shows the asymptotic optimality of our scheme. For $\nu = 1/2$, our constructions outperform Verkle commitments by about a factor of $2$ in terms of both the update information size and runtime, but makes use of larger public parameters.

==> meeting_notes.tex <==
Tentative Deadline: February 16

Meeting on Feb 1:

- Revised sections 2-3-4.
- Made the algorithms more precise, added pseudocode.
- Added table of comparison for the dichotomy of VCs.
- Thought about the lower bound:
-- If each node is allowed to do at most $\lambda$ bits of reading, then the proof update must contain $\lambda k$ bits of data per update.

- Discussion items:
-- (Misc. the royalty email about the slides) - ask them
-- (Misc. flashbots meeting) - read the post on the suave
-- (Financial Cryptography Reviews, updated version by February 10) 
-- Shall we add a section on RSA and bilinear accumulators? - table is sufficient
-- What other VC schemes can we add to the table? - done
-- Should we express complexity values in terms of group element sizes $|C|$, hash sizes $|H|$, number of group operations, hashes etc? - done
-- The upper bound: How can we formalize the argument above? Can we strengthen it to prove an upper bound on the tuples of functions $(g_1,g_2)$? 
-- ...

-ToDo items for introduction & evaluation.
-- Q: How are witnesses and update information propagated in Ethereum?
-- Q: Do we gain anything by reducing the size of the update information?
-- Q: Are witness updates envisioned by the protocol in this write-up doable for the light clients? 
-- Q: What about other VC schemes and operating points in terms of practical constraints?
-- Write evaluation
-- Write introduction

- ToDo: Add comments to the code - DONE

- ToDo: Should we add a dot to subsubsections? - DONE

- ToDos for Table:
-- Describe only the overhead over the changes. - DONE
-- Add the Merkle tree with homomorphic hash functions. - DONE
-- Third column: pre-processing data, global auxiliary data: linear and bilinear for KZG in the size of the pp, none for RSA. - DONE
-- Tree-based colunn -> get rid of, add a preprocessing column. - DONE
-- Express in terms of specific sizes - DONE

----------------------------------------
Discussion on the impossibility result:
----------------------------------------
Suppose the user is allowed to read only $\lambda$ bits of information.

-> If the update work is low, didn't read most of the messages, therefore, update message must be large since it must contain different data for different users for them to be able to update their proofs.

-> Suppose everyone is reading $N^{1-\nu}$ bits, yet, everyone eventually gets their new opening proofs, $N$ proofs in total.
-- User $i$ does not read $S_i$ of size $N-N^{1-\nu}$.
-- Then, $\cup_i [N] \backslash S_i = [N]$.
-- What is the minimum size of $S_i \cap S_j$ over all $i,j$.
---> Combinatorial problem!

--Thinking in terms of $N^\nu$ chunks of $N^{1-\nu}$ data.
--->My proof falls into a chunk.

Agenda for 2/13
------------------

1) Structure of the hash function used in the Merkle tree

(i) h(x, y) = h_x(x) * h_y(y) for some functions h_x(.) and h_y(.)

(ii) h(x_1 + x_2, y_1 + y_2) = h(x_1, y_1) * h(x_2, y_2) 

(iii) f(a_1 * ... * a_n) = f(a_1) + ... + f(a_n).

1.1) This determines the content of the evaluation section

- Evaluation of the KZG commitments

- Can we have any evaluation results for our VCs?

2) Lower bound write-up

3) Introduction layout

4) Submission

keygen gives pp
sequences not same

renyi entropy for random messages
renyi entropy compression result

Agenda for 4/6
------------------

1) Evaluation (Section 5.5)
- fix the typo
- elliptic curve operation cost:

ToDo items:
- Check out the library: https://github.com/supranational/blst.
- In the absence of good data, install benchmark and do the measurements locally: https://github.com/AlexiaChen/benchmarks-bls-libs

2) Appendix issue: can we assume N = poly(lambda)?

- No, but we are evaluating the overhead in the update information on top of the updated messages.

3) Theorem 1: Can we assume failure probability < e^(-lambda)?

- Yes, this is fine as stated in the Theorem.

4) How to restructure the paper? Verkle trees fall into the Merkle category.

- Current structure looks good. A conclusion might benefit the paper.

ToDo items:
- Box out Theorems for the update information and proof update time complexity within the text.

5) Introduction and the paper structure; section 4.3-1.2; proofs for the paper?

- Paper structure looks good.

6) Conference: We will submit to AFT.

7) Eth Denver problem: succinct clients for private chains!

ToDo items:
- Do more research on Penumbra's transaction operations.
- If these transaction operations are commutative, then it is possible to do 'ring' MPC, which makes communication complexity linear in the number of parties.
- FHE and general MPC with quadratic complexity are too expansive for Penumbra.
- Inviting Henry to seminar.

8) Next meeting, FC, summer and future plans

ToDo item:
- Ethresearch post on MEV capture attacks:
-- The validator can harness the proposer boost of the next slot by bribing the next validator to build on its block in order to reorg the relayer's block.
-- Think more about the potential attack; better exploits to reorg relayer blocks might be possible.

Agenda for 5/11
------------------

-- Financial Crypto Updates

1) Slides

2) Presentation: Limits on revocable proof systems, with implications for stateless blockchains. (Miranda Christ (Columbia University and a16z Crypto Research); Joseph Bonneau (New York University and a16z Crypto Research))

--> Main highlight seems to be a lower bound on how many witnesses must be updated when the global state size is small (namely, it is linear in k if the global state size is small).

In the case of Camacho and Hevia, we only care about the size of the update information.

-- Key management problem (from April 24)

1) The goal for the data structure is to support insertions and proofs of exclusion (technically, the data structure has to only show the exclusion of structured data, i.e., keys with higher versions; but I will ignore this for now. I think the following argument still applies). With such a data structure, it is possible to construct an accummulator that supports deletions. Thus, going forward, I will be working with an accummulator that supports deletions.

2) The server maintaining the data structure is not trusted. However, if it publishes conflicting commitments, clients can provably accuse the server. Therefore, we can assume that it only publishes a single commitment to the membership data. Then, the only fault that can be committed by the server is updating the commmitment incorrectly given the list of membership changes. I assume that this list is public. As an analogy, one can think of the commitment as the state root of a blockchain and the membership data as the blockchain ledger. Proving the 'validity' of the commitment in this paradigm can be done succinctly using a recursive SNARK. Hence, I will hereafter assume that all commitments are valid w.r.t. the membership data, and all users can verify this. Moreover, they can verify if a membership proof they received is valid by validating it against the valid commitment.

3) Without the concern for faulty servers, the main problem becomes reducing the storage cost and time complexity of generating membership proofs. We define 'update information' as the sequence of bits such that all proofs that were affected by the membership changes (during a pre-determined period) can be updated by observing these bits and the old data structure prior to the updates. Storage cost is the size of the update information, whereas time complexity is the time to generate a new proof given the old proof, old data structure and the update information.

4) I conjecture that a trade-off similar to the one in the paper (that is for the decentralized setting) holds here. The only difference is that here, the entity who tries to update its proof is the server itself, thus, has access to the internals of the old data structure besides the update information. Would this result in a smaller update information compared to the decentralized setting? I believe no; because such a result would mean that the mutual information between the 'old data structure' and the updated proofs is small, which would in turn imply too little entropy for the potential values of the updated proofs, i.e., a violation of the proof-binding property (defined in the paper). Indeed, the trie-based and algebraic constructions we have discussed on Monday support this observation.

5) For generalizing the analysis in the paper to the centralized setting, we should modify the setting for theorem 1 so that the clients, while updating their proofs, also have unlimited query access to the old data structure. 

-> I believe that proving theorem 1 under this model would be doable, if we can show that the mutual information between the new proofs and the old data structure is small (details are to be formalized).

--> All messages can be assumed independent. This assumption is needed not only to minimize the mutual information between the new proofs and the old data structure but also to minimize the mutual information between the unread messages and those that were read.

-- Problem about the Lower Bound

-> Can we say anything meaningful about the part of the update information beyond the published data when the update runtime is limited?

--> Yes, because the lower bound on the size of the update information is actually a lower bound on the 'part' of the update information beyond the published messages.

-> If runtime is not limited?

--> No.

-----------------------------------------
Suppose we did not have access to updated messages by the way of the blockchain.
What can we say about the updates themselves?

Since they are independent, they should be published? 

When $|\mathcal{M}| = \poly(\lambda)$, there is a proof and the above result is interesting!

When $|\mathcal{M}| = \exp(\lambda)$, what is a lower bound? If all messages, there is no asymptotic difference.

__________________________________________
------------------------------------------

ToDo items:

1) We should cite "Coniks Bringing Key Transperancy to End Users", ePrint 2014/1004 for the key management motivation.

2) We should cite "Limits on revocable proof systems, with implications for stateless blockchains". 
- What is the implications of this work?
--> It says that almost all proofs have to be updated in the case of our work. As a result, we answer how much effort it takes to update each proof and what update information size this implies.

- Highlight that our proof update time complexity is the complexity of the worst-off user; so we are bounding the complexity for all users!

3) Check the analysis for the $\log$ factor in the $\lambda k \log{N}$ expression. If this expression disappears, we might actually have an asymptotic gain in the update information size even in the case $|\mathcal{M}| = \exp(\lambda)$ and the updated messages are not accessible from the blockchain. 
In the paper, it must be highlighted that we can obtain the updated messages by the way of transactions in the blockchain.

4) Key management could be a motivation for this work. ToDo for Nusret: Add this discussion to the introduction and cite 2014/1004. 

Note: An important metric is minimizing the 'total' time to update the proofs. This needs more careful calculation.

Note: If I only maintain the tip of the tree, I would still have to use our lattice-based scheme.

While writing the motivation: the trade-off between storage (the tip of the tree, no access to the old data structures) and 'total' time to update the proofs (they are updated on the fly). 

5) Tangential Question: Can I efficiently prove that an accumulator is a subset of another accumulator (e.g., without using SNARKs)?

6) ToDo items for Nusret:

-- Obtaining the data for pairing calculations
-- Structuring the paper, in particular motivating the experimental results for Verkle trees
-- Notify Prof. Boneh after the updates.

<--> Meeting June 9 <-->

How should we reduce the number of pages?

IFCA copy-right form

Camera-ready version

Signature scheme

Cite the undergrad for Verkle trees

Table \hline

strongly homomorphic

linear merkle

homomorphic merkle tree
